Language-Preserving Reduction Rules for Block-Structured Workflow Nets

Process models are used by human analysts to model and analyse behaviour, and by machines to verify properties such as soundness, liveness or other reachability properties, and to compare their expressed behaviour with recorded behaviour within business processes of organisations. For both human and machine use, small models are preferable over large and complex models: for ease of human understanding and to reduce the time spent by machines in state space explorations. Reduction rules that preserve the behaviour of models have been defined for Petri nets, however in this paper we show that a subclass of Petri nets returned by process discovery techniques, that is, block-structured workflow nets, can be further reduced by considering their block structure in process trees. We revisit an existing set of reduction rules for process trees and show that the rules are correct, terminating, confluent and complete, and for which classes of process trees they are and are not complete. In a real-life experiment, we show that these rules can reduce process models discovered from real-life event logs further compared with rules that consider only Petri net structures.

==> sec4petrinets.tex <==
For Petri nets, superfluous model elements can be identified in silent transitions.
Such transitions can increase the complexity and the state space of models, making them potentially harder to understand for humans and more challenging to process for state-space-based techniques.
In this section, we introduce 7 reduction rules that remove silent transitions from any Petri net.
These rules are shown in Figure~\ref{fig:pn:rules}.
In this figure, the normal arcs are mandatory, the forbidden arcs are red, the optional arcs are dashed, the silent transitions are black and transitions that can be either labelled with an activity or silent are grey.
For each rule, if the left-hand pattern applies, the elements of the pattern can be reduced to the right-hand pattern.

Please note that most of these rules have been introduced in~\cite{DBLP:conf/bpm/PedroC16}; we formalise the rules and extend them: the FRT and SLT rules are extended and we discuss the implications of Petri nets with arc weights.

\subsection{The Rules}

	\def\impliesWidth{0.1cm}
	\def\ruleNameWidth{0.1\linewidth}
	\def\rulePictureWidth{0.35\linewidth}	
	\def\ruleConditionWidth{0.4\linewidth}
	\def\ruleEffectWidth{0.3\linewidth}

	\subsubsection{Fusion of Series Places.}
		There are two rules corresponding to the Fusion of Series Places rule~\cite{murata1989petri}: FSP1 and FSP2.
		
		\noindent
		\parbox{\ruleNameWidth}{FSP1} 
		\parbox[t]{\rulePictureWidth}{\input{rule-fsp1}}
		\parbox{\ruleConditionWidth}{Condition: $
			\begin{aligned}
				l(t) ={}& \tau\\
				p_1^{\bullet} ={}& \{t\}\\
				{}^{\bullet}t ={}& \{p_1\}\\
				t^{\bullet} ={}& \{p_2\}\\
				|(p_1, t)| ={}& 1\\
				|(t, p_2)| ={}& 1
			\end{aligned}$}
		\parbox{\ruleEffectWidth}{Effect: $
			\begin{aligned}
				{}^{\bullet}p' ={}& {}^{\bullet}p_1 \uplus {}^{\bullet}p_2\\
				p'^{\bullet} ={}& p_2^{\bullet}
			\end{aligned}$
		}
		
		\vspace{0.3cm}
		
		\noindent
		\parbox{\ruleNameWidth}{FSP2} 
		\parbox[t]{\rulePictureWidth}{\input{rule-fsp2}}
		\parbox{\ruleConditionWidth}{Condition: $
			\begin{aligned}
				l(t) ={}& \tau\\
				{}^{\bullet}p_2 ={}& \{t\}\\
				{}^{\bullet}t ={}& \{p_1\}\\
				t^{\bullet} ={}& \{p_2\}\\
				|(p_1, t)| ={}& 1\\
				|(t, p_2)| ={}& 1
			\end{aligned}$}
		\parbox{\ruleEffectWidth}{Effect: $
			\begin{aligned}
				{}^{\bullet}p' ={}& {}^{\bullet}p_1 \\
				p'^{\bullet} ={}& p_1^{\bullet} \uplus p_2^{\bullet}
			\end{aligned}$
		}

				If $p_1^{\bullet} = \{t\}$ and ${}^{\bullet}p_2 = \{t\}$, then both rules apply and have the same effect.				
		These two different conditions and consequently rules are necessary to prevent introducing looping behaviour.
		For instance, in the following Petri net fragment neither $p_1^{\bullet} = \{t\}$ nor ${}^{\bullet}p_2 = \{t\}$ hold.
		In this fragment, $a$ can be executed or skipped.
		However, if we would apply either FSP1 or FSP2, the result would allow $a$ to be executed repeatedly, thereby violating language equivalence:
		\begin{center}
			\input{rule-fsp-both}
		\end{center}
		
		Both rules only apply to singular edges, as a transition $t$ with multiple in- and outgoing edges provides synchronisation between the tokens in $p_1$, which would be lost by applying either rule.
		For instance, in the following process fragment the trace $a, c, b$ is introduced by applying either of the rules FSP1 or FSP2.
		\begin{center}
			\input{rule-fsp-multiplicities}
		\end{center}
		
	\subsubsection{Fusion of Series Transitions.}
		Similarly, there are two rules corresponding to the Fusion of Series Transitions rule~\cite{murata1989petri}: FST1 and FST2.
		
		\noindent
		\parbox{\ruleNameWidth}{FST1} 
		\parbox[t]{\rulePictureWidth}{\input{rule-fst1}}
		\parbox{\ruleConditionWidth}{Condition: $
			\begin{aligned}
				l(t_1) ={}& \tau\\
				t_1^{\bullet} ={}& \{p\}\\
				{}^{\bullet}p ={}& \{t_1\}\\
				p^{\bullet} ={}& \{t_2\}\\
				|(t_1, p)| ={}& x |(p, t_2)|
			\end{aligned}$}
		\parbox{\ruleEffectWidth}{Effect: $
			\begin{aligned}
				l(t') ={}& l(t_2)\\
				{}^{\bullet}t' ={}& x {}^{\bullet}t_1 \uplus {}^{\bullet}t_2\\
				t'^{\bullet} ={}& t_2^{\bullet}
			\end{aligned}$
		}
		
		\vspace{0.3cm}
		
		\noindent
		\parbox{\ruleNameWidth}{FST2} 
		\parbox[t]{\rulePictureWidth}{\input{rule-fst2}}
		\parbox{\ruleConditionWidth}{Condition: $
			\begin{aligned}
				l(t_2) ={}& \tau\\
				{}^{\bullet}t_2 ={}& \{p\}\\
				{}^{\bullet}p ={}& \{t_1\}\\
				p^{\bullet} ={}& \{t_2\}\\
				|(t_1, p)| ={}& |(p, t_2)|
			\end{aligned}$}
		\parbox{\ruleEffectWidth}{Effect: $
			\begin{aligned}
				l(t') ={}& l(t_1)\\
				{}^{\bullet}t' ={}& {}^{\bullet}t_1\\
				t'^{\bullet} ={}& t_1^{\bullet} \uplus t_2^{\bullet}
			\end{aligned}$
		}
		
		If $t_1^{\bullet} = \{p\}$, ${}^{\bullet}t_2 = \{p\}$, $l(t_1) = \tau$ and $l(t_2) = \tau$ then both rules apply and have the same effect.
		
		\todo{multiplicities}
		\begin{center}
			\input{rule-fst-multiplicities}
		\end{center}
	
	\subsubsection{Fusion of Redundant Transitions.}
		Two silent transitions that are overlapping in cause and effect are redundant to one another.
		
		\noindent
		\parbox{\ruleNameWidth}{FRT} 
		\parbox[t]{\rulePictureWidth}{\input{rule-frt}}
		
		\hspace*{\fill}\parbox{\ruleConditionWidth}{Condition: $
			\begin{aligned}
				l(t_1) ={}& \tau\\
				l(t_2) ={}& \tau\\
				{}^{\bullet}t_1 ={}& {}^{\bullet}t_2\\
				t_1^{\bullet} ={}& t_2^{\bullet}
			\end{aligned}$}
		\parbox{\ruleEffectWidth}{Effect: $
			\begin{aligned}
				l(t') ={}& \tau\\
				{}^{\bullet}t' ={}& {}^{\bullet}t_1\\
				t'^{\bullet} ={}& t_1^{\bullet}
			\end{aligned}$
		}
		
		There can be an arbitrary number of places $p_1$ and $p_2$, as long as $t_1$ and $t_2$ have the same incoming and outgoing edges to these places.

\subsection{Analysis}
	For all the rules, a careful assessment reveals that they preserve the language of the model.
	Please note that no labelled transition, that is, a transition with an attached activity, is ever removed.
	
	The rules FSPI, FSPII and FRP reduce the number of places in the model, thus the number of states in the state space of the model, while the other rules reduce the number of transitions in the model, thus the possible steps in the state space.
	Consequently:
	
	\begin{corollary}
		repeated application of the Petri net rules (Figure~\ref{fig:pn:rules}) is terminating.
		Only if the elements used in the rules are distinct.
	\end{corollary}
	
	\begin{figure}
		\begin{subfigure}[b]{\linewidth}
			\centering
			
			\caption{Fusion of Redundant Transitions (FRT). Condition: $t_1^{\cdot} = t_2^{\cdot}$ and ${}^{\cdot}t_1 = {}^{\cdot}t_2$.}
		\end{subfigure}
		\begin{subfigure}[b]{\linewidth}
			\centering
			\begin{tikzpicture}
				\node [draw, fill, minimum height=0.5cm] (t1) {};
				\node [draw, circle, right of=t1, yshift=-0.3cm, label=below:$p_2$] (p1) {};
				\node [draw, circle, right of=t1, yshift=0.3cm, label=$p_1$] (p2) {};
				\node [draw, fill, minimum height=0.5cm, right of=p1, yshift=0.3cm] (t2) {};
				\draw [->] (t1) to (p1);
				\draw [->] (p1) to (t2);
				\draw [->] (t1) to (p2);
				\draw [->] (p2) to (t2);
				
				\draw [<-, dashed] (t1) to ++(-0.3cm,0.4cm);
				\draw [->, dashed] (t1) to ++(0.3cm,-0.4cm);
				\draw [<-, red] (p1) to ++(-0.3cm,0.4cm);
				\draw [->, red] (p1) to ++(0.3cm,-0.4cm);
				\draw [<-, red] (p2) to ++(-0.3cm,0.4cm);
				\draw [->, red] (p2) to ++(0.3cm,-0.4cm);
				\draw [<-, dashed] (t2) to ++(-0.3cm,0.4cm);
				\draw [->, dashed] (t2) to ++(0.3cm,-0.4cm);
				
				\node [right of=t2] (a) {$\Rightarrow$};
				
				\node [draw, fill, minimum height=0.5cm, right of=a] (t3) {};
				\node [draw, circle, right of=t3] (p3) {};
				\node [draw, fill, minimum height=0.5cm, right of=p3] (t4) {};
				
				\draw [->] (t3) to (p3);
				\draw [->] (p3) to (t4);
				
				\draw [<-, dashed] (t3) to ++(-0.3cm,0.4cm);
				\draw [->, dashed] (t3) to ++(0.3cm,-0.4cm);
				\draw [<-, dashed] (t4) to ++(-0.3cm,0.4cm);
				\draw [->, dashed] (t4) to ++(0.3cm,-0.4cm);
			\end{tikzpicture}
			\caption{Fusion of Redundant Places (FRP). Condition: $p_1^{\cdot} = p_2^{\cdot}$ and ${}^{\cdot}p_1 = {}^{\cdot}p_2$.}
		\end{subfigure}
		\begin{subfigure}[b]{\linewidth}
			\centering
			\begin{tikzpicture}
				\node [draw, circle] (p1) {};
				\node [draw, fill, minimum height=0.5cm, right of=p1, label=$t$] (t) {};
				\node [draw, circle, right of=t] (p2) {};
				
				\draw [->, bend left, bend angle=15] (p1) to (t);
				\draw [->, bend left, bend angle=15] (t) to (p1);
				\draw [->, bend left, bend angle=15, dashed] (p2) to (t);
				\draw [->, bend left, bend angle=15, dashed] (t) to (p2);
			\end{tikzpicture}
			\caption{Removal of Self-Loop Transitions (SLT). Condition: $t^{\cdot} = {}^{\cdot}t$.}
		\end{subfigure}
		\caption{Reduction rules for Petri nets. Optional arcs are dashed; forbidden arcs are red. Black transitions are silent and gray transitions are either labelled or silent.}
		\label{fig:pn:rules}
	\end{figure}
